Invariants of moduli spaces of stable sheaves on ruled surfaces

We compute Betti numbers of the moduli spaces of arbitrary rank stable sheaves on ruled surfaces. Our result generalizes the formula of Goettsche for rank one sheaves and the formula of Yoshioka for rank two sheaves. It also confirms the conjecture of Manschot for arbitrary rank sheaves on the Hirzebruch surfaces.

==> command.tex <==
%%%% abbreviations %%%%
\RequirePackage{amsmath,amsthm,amssymb,xspace}

\def\makedef#1#2{\expandafter\gdef\csname#1\endcsname{#2}}
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}} 				% \dmat\name{commands}
\def\dmata#1#2{\makedef{#1}{\mat{#2}}}	% \dmata{name}{commands}
\def\dmatb#1{\dmat#1} %open {} for \dmat
\def\makelet#1#2{\expandafter\let\csname#1\expandafter\endcsname\csname#2\endcsname}
\def\redefmath#1{\makelet{temp@#1}{#1}\dmata{#1}{\csname temp@#1\endcsname}}

\def\listdo#1#2{\gdef\listproc{#1}\listdox#2,xxx,}%#1-procedure,#2-list
\def\listend{xxx}
\def\listdox#1,{\def\temp{#1}\ifx\temp\listend\relax\else\listproc{#1}\expandafter\listdox\fi}


%%%% Standard structures and Calligraphic letters, Gothic letters %%%%
\def\defbb#1{\dmata{b#1}{\mathbb{#1}}}
%\dmata{c#1}{\mathbb{#1}}}%usage \bA
\def\defcal#1{\dmata{c#1}{\mathcal{#1}}\dmata{l#1}{\mathcal{#1}}}	% usage \cA
\def\deffrak#1{\dmata{f#1}{\mathfrak{#1}}} % usage \ga,\gA
\def\defserif#1{\dmata{s#1}{\mathsf{#1}}}
\def\defbf#1{\dmata{bf#1}{\mathbf{#1}}}
\def\defroman#1{\dmata{r#1}{\mathrm{#1}}}
\def\defall#1{\defbb{#1}\defcal{#1}\deffrak{#1}\defserif{#1}\defbf{#1}\defroman{#1}}
\listdo\defall{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\def\bbm{
\RequirePackage{bbm}
\dmat\bk{\mathbbm{k}}
%\def\defbbm##1{\dmata{b##1}{\mathbbm{##1}}}		% usage \cA
%\listdo\defbbm{k}
}

%%%% Gothic/Fraktur Letters %%%%%
\listdo\deffrak{a,b,c,d,f,h,j,k,m,n,o,p,q,s,t,u,v,w,x,y,z}
%\ge=>=, \gg=>>, \ggg=>>>, \gl=lie algebra, \gr=graded 
\dmat\fg{\mathfrak g}
\dmat\fe{\mathfrak e}
\dmat\fl{\mathfrak l}
\dmat\fr{\mathfrak r}
\def\g{\fg}
\def\gge{\fe}
\def\ggl{\fl}

%%%%% Greek letters %%%%%
\dmat\al\alpha
\dmat\be\beta
\dmat\ga\gamma
\dmat\Ga\Gamma
\dmat\de\delta
\dmat\De\Delta
\dmat\eps\varepsilon
\dmat\Eps\lE
\dmat\epsi\epsilon
\dmat\hi\chi
\dmat\kapa\kappa
\dmat\kp\kappa
\dmat\ksi\xi
\dmat\La\Lambda
\dmat\la\lambda
\dmat\Nabla\bigtriangledown
\dmat\Na\nabla
\dmat\Om\Omega
\dmat\om\omega
\dmat\vi\varphi
\dmat\si\sigma
\dmat\Si\Sigma
\dmat\ze\zeta
\dmat\te\theta
\dmat\Te\Theta
\dmat\Tau{\mathcal{T}}
\listdo\redefmath{eta,xi,mu,nu,Phi,Psi,psi,pi,rho}
\dmat\ta{\tau}


%%%% Functions %%%%%
\def\DMO#1#2{\dmat#1{\operatorname{#2}}}  % \DMO\name{command}
\def\oper#1{\dmata{#1}{\operatorname{#1}}}
\def\DMOx{\DeclareMathOperator*}
\def\operx#1{\expandafter\DMOx\csname#1\endcsname{#1}}

\listdo\oper{Hom,RHom,Ext,End,Aut,Fun,Tor,ext,hom}
\DMO\lHom{\lH\mathit{om}}
\DMO\lEnd{\lE\mathit{nd}}
\DMO\lExt{\lE\mathit{xt}}

\listdo\oper{Ob,Mor,Arr,im,coim,coker}
\listdo\oper{Id,id,add,ind,pro,Map,Maps,Iso,Isom,Ind,Bun,Loc}
\listdo\oper{Sch,Var,Cat,Set,Ab,Alg,Ring,Mon,Vect,sSet,sCat,mod}
\listdo\oper{Presh,Sh,Per,Perf,Coh,coh,QCoh}
\listdo\oper{Rep,Cor,Mod,rad,soc,ann,pd}
\listdo\oper{Spec,Specm,Max,Proj,supp,Pic,Div,Jac,Fitt}
\listdo\oper{Hilb,Quot,Flag,Grass,Higgs,Hitch}
\listdo\oper{cone,Tw,rk,codim,cov,sgn,td,Gr,gr,ch,cl}
\listdo\oper{GL,PGL,SL,PU,SO,SU,Sp,Mat,spin}
\listdo\oper{HMod,Ho,sk,cosk,}
\listdo\oper{Der,Ad,ad}
\listdo\oper{Exp,Log,Pow,pow,Sym}
\listdo\oper{diag,Gal,tr,Tr,Is,Hol,Res,Ind,irr,Irr,mult,wt,hd,face,Eig,Li,St,Im,Re,crit,per,nil}
\listdo\oper{Diff,Fr,Perv,res,Aff,FT,Sol,DR}

%%%%Operads
\listdo\oper{Gerst,Lie,Com,Ass,Pois,Hoch,Def}

\dmat\gl{\mathfrak{gl}}
\dmat\sl{\mathfrak{sl}}
\dmat\so{\mathfrak{so}}
\dmat\su{\mathfrak{su}}
\def\Hig{\Higgs}
\def\Hit{\Hitch}
\def\Gras{\Grass}
\dmat\cosimp{{\bf\De}^\op} %cosimplexes
\dmat\simp{\bf\De} %simplexes

\def\ilim{\varprojlim} %inverse limit
\def\plim{\ilim}
\def\dlim{\varinjlim} %direct limit
\listdo\operx{colim,hocolim,holim}

%%%% Non-standard (compatibility issues) %%%%
\def\deop{\cosimp}
\DMO{\har}{char}
\DMO{\height}{ht} %
\DMO{\der}{Der}
\DMO{\coder}{Coder}
\DMO{\rank}{rk}
\DMO{\spec}{Spec}
\DMO{\Qcoh}{QCoh}
\DMO{\coalg}{Coalg}
\dmat\Ch{\mathbf{Ch}} %chain complexes

%%%%% symbols %%%%%%
\dmat\Gm{{\bG_{\mathrm m}}}
\def\GIT{/\!\!/}
\def\norm#1{\mat{\lVert#1\rVert}}
\def\n#1{\mat{\lvert#1\rvert}}
\def\nn#1{\mat{\lVert#1\rVert}}
\def\lrb#1{\left(#1\right)}
\dmat\dd{\partial}
\def\iso{\simeq}
\def\ts{\otimes}
%\def\sqt{\boxtimes}
\def\lts{\mat{\stackrel{\bf L}\otimes}}
\def\tl#1{\mat{\tilde{#1}}}
\def\wtl#1{\mat{\widetilde{#1}}}
\def\what#1{\mat{\widehat{#1}}}
\def\conjug#1{\overline{#1}}
%\def\sb{\subset}
\def\sbe{\subseteq}
\def\sbne{\varsubsetneq}
\def\sbneq{\sbne}
\def\spe{\supseteq}
%\def\sp{\supset}
\dmat\imp\Rightarrow
\dmat\iff\Leftrightarrow
%\def\xarr#1{\xrightarrow{#1}}
\def\sd{\rtimes} %semidirect product
\def\xx{\times}
\def\ox{\otimes}
\def\bs{\backslash}
\def\ms{\backslash} %minus set
\def\es{\emptyset}
\dmat\pt{\mathbf {pt}} %point
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{\mbox{(\!(}#1\mbox{)\!)}} %formal Laurent series ((#1))
\def\brc#1{\{#1\}}
\def\dbrc#1{\{\hspace{-3.1pt}\{#1\}\hspace{-3.1pt}\}}
%\def\pser#1{\Lbrack#1\Rbrack}
%\def\lser#1{\Lparen #1 \Rparen}
\def\llser#1{\llparenthesis #1 \rrparenthesis}
\def\lpoly{\pser}% reverse compatibility
\def\fser{\lser}% reverse compatibility
\def\vac{\mat{\mathbf{1}}}%vacuum vector
\def\partof{\vdash}
\dmat\half{\frac12}
\def\oh{\half} %one half
\def\bop{\bigoplus}
\def\bts{\bigotimes}
\def\udim{\lb\dim}
\makeatletter
\@ifpackageloaded{bbm}
{\def\one{\mathbbm{1}}}
{\def\one{\mathbf{1}}}
\makeatother

%%% sub/superscripts
\def\m{{-1}}
\def\inv{^{-1}}
\def\dual{^\vee}
\def\tors{{\rm tors}}
\def\st{{\mathrm{st}}}
\def\sst{{\rm sst}}
\def\orb{{\rm orb}}
\def\nil{\mathrm{nil}}
\def\cond#1#2{\left.#1\right|_{#2}}  %f|_{x=a}
%\def\refl{^{\vee\vee}}
\def\op{{\rm op}}
\def\red{{\rm red}}
\def\tw{{\rm tw}}
\def\et{{\rm et}}
\def\vir{{\rm vir}}
%\def\dual{{\!\!\:\text{\textasciicaron}}} %requires textcomp
%\def\refl{^{\vee\vee}} %was called refl before


%%%% Structures %%%%%%
\def\rbr#1{\left(#1\right)}
\def\qbinom#1#2{\mat{\genfrac{[}{]}{0pt}{}{#1}{#2}}}  %q-binomial
\def\ang#1{\mat{\left\langle #1\right\rangle}}
\def\angs#1#2{\mat{\left\langle #1 \mid #2\right\rangle}}
\def\set#1{\mat{\{#1\}}}
\def\sets#1#2{\mat{\{#1\mid#2\}}}
\def\vect#1{\mat{({}\begin{smallmatrix}#1\end{smallmatrix}{})}}
\def\smat#1{\mat{\left(\begin{smallmatrix}#1\end{smallmatrix}\right)}}
\def\case#1{\begin{cases}#1\end{cases}}

%%%% Arrows %%%%%
\def\emb{\hookrightarrow}
\def\mto{\mapsto}
\def\arr{\futurelet\test\arrtest}
\def\arrtest{\ifx^\test\expandafter\arra\else\expandafter\tempto\fi}
\def\arra^#1{\xrightarrow{#1}}
\let\tempto\to
\def\to{\arr}
%\def\ar{\arr}
\def\rrarr{\pile{\rTo\\ \rTo}}
\def\lrarr{\pile{\rTo\\ \lTo}}   
\def\ot{\leftarrow}

%%%%% Theorems %%%%%%
\newcounter{nthr} %auxiliary counter
\numberwithin{nthr}{section}
\let\theHnthr\thenthr

%solves a problem with hyperref, Heiko <oberdiek@ruf.uni-freiburg.de>
%a different solution: option hypertexnames=false in hyperref

\def\theorems{
\theoremstyle{plain}
\newtheorem{thr}[nthr]{Theorem}
\newtheorem{prp}[nthr]{Proposition}
\newtheorem{lmm}[nthr]{Lemma}
\newtheorem{crl}[nthr]{Corollary}
\newtheorem{clm}[nthr]{Claim}
\newtheorem{conj}{Conjecture}
\newtheorem{rmr}[nthr]{Remark}
\theoremstyle{definition}
\newtheorem{dfn}[nthr]{Definition}
\newtheorem{exm}[nthr]{Example}
\theoremsFull
}

\def\theoremsFull{
\theoremstyle{plain}
\newtheorem{theorem}			[nthr]{Theorem}
\newtheorem{proposition}	[nthr]{Proposition}
\newtheorem{lemma}				[nthr]{Lemma}
\newtheorem{corollary}		[nthr]{Corollary}
\newtheorem{claim}				[nthr]{Claim}
\newtheorem{conjecture}   			{Conjecture}
\newtheorem{remark}       [nthr]{Remark}
\theoremstyle{definition}
\newtheorem{definition}   [nthr]{Definition}
\newtheorem{example}      [nthr]{Example}
}

\def\useElsart{
\def\rqed{\hfill{ }\qed}
\newenvironment{proof}[1][PROOF.]{\begin{pf*}{##1}}{\rqed\end{pf*}}
\def\thr{\thm}
\def\prp{\prop}
\def\lmm{\lem}
\def\crl{\cor}
\def\clm{\claim}
%\def\conj}{\conj}
\def\dfn{\defn}
\def\rmr{\rem}
\def\exm{\exmp}}

\def\useSpringer{
\def\thr{\theorem}
\def\prp{\proposition}
\def\lmm{\lemma}
\def\crl{\corollary}
\def\conj{\conjecture}
\def\dfn{\definition}
\def\rmr{\remark}
\def\exm{\example}}

\def\theoremsSpringer{
\theoremsFull
}

\def\theoremsElsevier{
%prop,thm,lem,cor,conj,defn,rem,exmp,claim,note
\theoremstyle{plain}
\newtheorem{thm}    [nthr]{Theorem}
\newtheorem{prop}   [nthr]{Proposition}
\newtheorem{lem}    [nthr]{Lemma}
\newtheorem{cor}    [nthr]{Corollary}
\newtheorem{conj}   [nthr]{Conjecture}
\theoremstyle{definition}
\newtheorem{defn}   [nthr]{Definition}
\newtheorem{rem}    [nthr]{Remark}
\newtheorem{exmp}   [nthr]{Example}}


%%%%%%%%%%%%%%%%%%Margin notes \rem{}%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifrem\remtrue
\def\rem#1{\ifrem\marginpar{\raggedright\footnotesize #1}\fi}

%%%% different %%%%%
\dmat\ainf{A_\infty}
\def\br{\linebreak}
\def\lb#1{\mat{\underline{#1}}} %lower bar
\def\ub#1{\mat{\overline{#1}}}  %upper bar
%\def\over#1#2{\mat{\stackrel #2#1}} % #2 over #1
\def\over#1#2{\mat{\substack{#1\\#2}}} % #1 over #2
\def\overst#1#2{\mat{\substack{#1\\#2}}} % #1 over #2
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
\def\ie{i.e.\ }
\def\eg{e.g.\ }
\def\cf{cf.\ }

%%%%%%%%%%%%%%%%%%%%%% Knots
%Defaults: linewidth=.8pt, arrowwidth=1.5pt 2 that is width=1.5+2*.8=3.1pt, length=1.4*width=4.3pt, inset=.4*length=

%\def\psar{\psline{-}(-.1,.1)(0,0)(-.1,-.1)}
%\def\psar{\pspolygon[fillstyle=solid,fillcolor=black,unit=30\pslinewidth](0,0)(-.14,-.05)(-.084,0)(-.14,.05)}
%\def\psar{\pspolygon[fillstyle=solid,fillcolor=black,yunit=1.2pt,xunit=1.68pt](0,0)(-1,-.5)(-.6,0)(-1,.5)}
\def\psar{\psline{->}(-.05,0)(0,0)}
\def\psa#1#2{\aput(#1){#2}\lput{:0}(#1){\psar}}
\def\psb{\psa{.5}{}}
\def\nm#1{[name=#1]}
\def\psm#1{\psset{arrows=->,nodesep=2pt,colsep=1cm,rowsep=1cm}\begin{psmatrix}#1\end{psmatrix}}


\def\pst#1{\begin{pspicture}#1\end{pspicture}}


%%%%%%%%%%% some knot symbols
%\RequirePackage{pstricks}
\makeatletter
\def\symbolBox#1#2{%half size,code
\pssetlength\pst@dima{-#1}
\psaddtolength\pst@dima{.75ex}
\psset{unit=#1,shift=\pst@dima,linewidth=.075,arrows=-}
\pst{(2,2)#2}}
\makeatother

\def\dsmb#1#2{\gdef#1{\symbolBox{1ex}{#2}}}

\dsmb\doublepoint{
\psline{->}(2,0)(0,2)\psline{->}(0,0)(2,2)\psdot(1,1)}
\dsmb\overcrossing{
\psline{->}(0,0)(2,2)\psline{->}(.8,1.2)(0,2)\psline{-}(2,0)(1.2,.8)}
\dsmb\undercrossing{
\psline{->}(2,0)(0,2)\psline{->}(1.2,1.2)(2,2)\psline{-}(0,0)(.8,.8)}
\dsmb\crossing{\psline{->}(2,0)(0,2)\psline{->}(0,0)(2,2)}
\dsmb\Ucrossing{\psline(2,0)(0,2)\psline(0,0)(2,2)}
\dsmb\Uovercrossing{
\psline{-}(0,0)(2,2)\psline{-}(.8,1.2)(0,2)\psline{-}(2,0)(1.2,.8)}
\dsmb\Uundercrossing{
\psline{-}(2,0)(0,2)\psline{-}(1.2,1.2)(2,2)\psline{-}(0,0)(.8,.8)}
\dsmb\smoothing{
\psline[linearc=1]{->}(0,0)(1,1)(0,2)\psline[linearc=1]{->}(2,0)(1,1)(2,2)}
\dsmb\hsmoothing{
\psline[linearc=1]{->}(0,0)(1,1)(2,0)\psline[linearc=1]{->}(0,2)(1,1)(2,2)}
\dsmb\Usmoothing{
\psline[linearc=1]{-}(0,0)(1,1)(0,2)\psline[linearc=1]{-}(2,0)(1,1)(2,2)}
\dsmb\Uhsmoothing{
\psline[linearc=1]{-}(0,0)(1,1)(2,0)\psline[linearc=1]{-}(0,2)(1,1)(2,2)}
\dsmb\unknot{\pscircle(1,1){1}}
\dsmb\fourwheel{
\SpecialCoor\pscircle(1,1){.7}\rput(1,1){\psline(.7;45)(1,1)\psline(.7;135)(-1,1)\psline(.7;225)(-1,-1)\psline(.7;-45)(1,-1)}}
\dsmb\twowheel{
\pscircle(1,1){.5}\psline(0,1)(.5,1)\psline(2,1)(1.5,1)}
\dsmb\fourinwheel{
\SpecialCoor\pscircle(1,1){1}\rput(1,1){\psline(.5;45)(1;45)\psline(.5;135)(1;135)\psline(.5;225)(1;225)\psline(.5;-45)(1;-45)}}
\dsmb\IGraph{
\psline(0,0)(1,.4)(2,0)\psline(0,2)(1,1.6)(2,2)\psline(1,.4)(1,1.6)}
\dsmb\HGraph{
\psline(0,0)(.4,1)(0,2)\psline(2,0)(1.6,1)(2,2)\psline(.4,1)(1.6,1)}
\dsmb\XGraph{
\psline(0,0)(2,2)\psline(2,0)(0,2)\psline(.5,.5)(1.5,.5)}
\dsmb\SGraph{
\psline(0,2)(1,1.2)(2,2)\psline(1,0)(1,1.2)\psline[linewidth=.2](0,0)(2,0)}
\dsmb\TGraph{
\psline(0,2)(.5,0)\psline(2,2)(1.5,0)\psline[linewidth=.2](0,0)(2,0)}
\dsmb\UGraph{
\psline(0,2)(1.5,0)\psline(2,2)(.5,0)\psline[linewidth=.2](0,0)(2,0)}
\dsmb\YGraph{\psline(0,2)(1,1.2)(2,2)\psline(1,0)(1,1.2)}
\dsmb\HSaddle{\psline[linearc=1](0,0)(1,1)(0,2)\psline[linearc=1](2,0)(1,1)(2,2)\psline(.6,1)(1.4,1)}
\dsmb\ISaddle{\psline[linearc=1](0,0)(1,1)(2,0)\psline[linearc=1](0,2)(1,1)(2,2)\psline(1,.6)(1,1.4)}


\def\showKnotSymbols{
\begin{table}
\begin{tabular}{|l|c|}
\hline
\tt{\string\crossing}&\crossing\\
\tt{\string\overcrossing}&\overcrossing\\
\tt{\string\undercrossing}&\undercrossing\\
\tt{\string\doublepoint}&\doublepoint\\
\tt{\string\Ucrossing}&\Ucrossing\\
\tt{\string\Uovercrossing}&\Uovercrossing\\
\tt{\string\Uundercrossing}&\Uundercrossing\\
\tt{\string\smoothing}&\smoothing\\
\tt{\string\hsmoothing}&\hsmoothing\\
\tt{\string\Usmoothing}&\Usmoothing\\
\tt{\string\Uhsmoothing}&\Uhsmoothing\\
\tt{\string\unknot}&\unknot\\
\tt{\string\twowheel}&\twowheel\\
\tt{\string\fourwheel}&\fourwheel\\
\tt{\string\fourinwheel}&\fourinwheel\\
\tt{\string\IGraph}&\IGraph\\
\tt{\string\HGraph}&\HGraph\\
\tt{\string\XGraph}&\XGraph\\
\tt{\string\SGraph}&\SGraph\\
\tt{\string\TGraph}&\TGraph\\
\tt{\string\UGraph}&\UGraph\\
\tt{\string\YGraph}&\YGraph\\
\tt{\string\ISaddle}&\ISaddle\\
\tt{\string\HSaddle}&\HSaddle\\
\hline
\end{tabular}
\caption{Knot symbols}
\end{table}}

%%%%%%citations
\makeatletter
\def\rf{\@ifnextchar[{\rf@e}{\rf@b}}
\def\rf@b#1{\def\rf@y{#1}%
\@ifnextchar[{\rf@d\rf@y}{\rf@e\rf@y}}
\def\rf@d#1[#2]{\rf@e[#2]#1}
\let\rf@e\cite
%\def\cite{\rf}
\makeatother


\endinput


